Performance of QUIC Implementations Over Geostationary Satellite Links

QUIC was recently standardized as RFC 9000, but the performance of QUIC over geostationary satellite links is problematic due to the non-applicability of Performance Enhancing Proxies. As of today, there are more than a dozen of different QUIC implementations. So far performance evaluations of QUIC over satellite links were limited to specific QUIC implementations. By deploying a modified version of the IETF QUIC-Interop-Runner, this paper evaluates the performance of multiple QUIC implementations over multiple geostationary satellite links. This includes two emulated ones (with and without packet loss) and two real ones. The results show that the goodput achieved with QUIC over geostationary satellite links is very poor in general, and especially poor when there is packet loss. Some implementations fail completely and the performance of the other implementations varies greatly. The performance depends on both client and server implementation.

==> img/tikz/latex-common/cmds.tex <==
\newcommand{\bps}{\bit\per\second}
\newcommand{\kbps}{\kilo\bit\per\second}
\newcommand{\mbps}{\mega\bit\per\second}
\newcommand{\gbps}{\giga\bit\per\second}
\newcommand{\tbps}{\tera\bit\per\second}
\newcommand{\kb}{\kilo\byte}
\newcommand{\mb}{\mega\byte}
\newcommand{\gb}{\giga\byte}
\newcommand{\kib}{\kibi\byte}
\newcommand{\mib}{\mebi\byte}
\newcommand{\gib}{\gibi\byte}
\newcommand{\tib}{\tera\byte}

\def\lr/{\textsc{LongRTT}}
\def\g/{\textsc{Goodput}}
\def\sat/{\textsc{Sat}}
\def\satl/{\textsc{SatLoss}}
\def\eut/{\textsc{Eutelsat}}
\def\astra/{\textsc{Astra}}
\def\crosstraffic/{\textsc{CrossTraffic}}

\def\pcap/{Pcap}
\def\pcapng/{Pcap NG}
\def\keylog/{key-log}
\def\Keylog/{Key-log}
\def\netem/{NetEm}
\def\dummynet/{dummynet}
\def\Nsthree/{\mbox{ns-3}}
\def\nsthree/{\mbox{ns-3}}
\def\Wireshark/{Wireshark}
\def\wireshark/{Wireshark}
\def\Tshark/{TShark}
\def\tshark/{TShark}
\def\Pyshark/{Pyshark}
\def\pyshark/{pyshark}
\def\Tcpdump/{Tcpdump}
\def\tcpdump/{tcpdump}
\def\Qlog/{qlog}
\def\qlog/{qlog}
\def\Qvis/{qvis}
\def\qvis/{qvis}
\def\Python/{Python}
\def\python/{\Python/}
\def\dockerpy/{docker-py}
\def\Docker/{Docker}
\def\docker/{\Docker/}
\def\Doco/{\Docker/ Compose}
\def\doco/{\Doco/}

\def\PC/{\acs{PC}}
\def\IoT/{\acs{IoT}}
\def\URL/{\acs{URL}}

\def\IETF/{\acs{IETF}}
\def\RFC/{\acs{RFC}}

\def\SATCOM/{\acs{SATCOM}}

\def\RTT/{\acs{RTT}}
\def\IP/{\acs{IP}}
\def\ICMP/{\acs{ICMP}}
\def\UDP/{\acs{UDP}}
\def\TCP/{\acs{TCP}}
\def\SCTP/{\acs{SCTP}}
\def\WebRTC/{\acs{WebRTC}}
\def\QUIC/{QUIC}
\def\gQUIC/{gQUIC}
\def\HTTP/{\acs{HTTP}}
\def\TLS/{\acs{TLS}}
\def\LAN/{\acs{LAN}}
\def\VPN/{\acs{VPN}}
\def\DNS/{\acs{DNS}}
\def\MASQUE/{\acs{MASQUE}}

\def\BBR/{\acs{BBR}}
\def\BBRv2/{\BBR/v2}
\def\BIC/{BIC}
\def\CUBIC/{CUBIC}
\def\Reno/{Reno}
\def\NewReno/{NewReno}
\def\pico/{pico}

\def\SYN/{\texttt{SYN}}
\def\SYNs/{\texttt{SYNs}}
\def\ACK/{\texttt{\acs{ACK}}}
\def\ACKs/{\texttt{\acsp{ACK}}}
\def\NACK/{\texttt{NACK}}
\def\FIN/{\texttt{FIN}}
\def\STREAM/{\texttt{STREAM}}

\def\aioquic/{\textit{aioquic}}
\def\chrome/{\textit{chrome}}
\def\kwik/{\textit{kwik}}
\def\lsquic/{\textit{lsquic}}
\def\msquic/{\textit{msquic}}
\def\mvfst/{\textit{mvfst}}
\def\neqo/{\textit{neqo}}
\def\nginx/{\textit{nginx}}
\def\ngtcp/{\textit{ngtcp2}}
\def\picoquic/{\textit{picoquic}}
\def\quant/{\textit{quant}}
\def\quicgo/{\textit{quic-go}}
\def\quiche/{\textit{quiche}}
\def\quicly/{\textit{quicly}}
\def\xquic/{\textit{xquic}}

\def\Aioquic/{\textit{Aioquic}}
\def\Chrome/{\textit{Chrome}}
\def\Kwik/{\textit{Kwik}}
\def\Lsquic/{\textit{Lsquic}}
\def\Msquic/{\textit{Msquic}}
\def\Mvfst/{\textit{Mvfst}}
\def\Neqo/{\textit{Neqo}}
\def\Nginx/{\textit{NGINX}}
\def\Ngtcp/{\textit{Ngtcp2}}
\def\Picoquic/{\textit{Picoquic}}
\def\Quant/{\textit{Quant}}
\def\Quicgo/{\textit{Quic-go}}
\def\Quiche/{\textit{Quiche}}
\def\Quicly/{\textit{Quicly}}
\def\Xquic/{\textit{Xquic}}

% FFUUU!!!
\newcommand{\acps}[1]{\acsp{#1}}

\newcommand{\makeunit}[1]{{\mdseries\color{aluminium6}{$[\si{#1}]$}}}


==> img/tikz/latex-common/setup.tex <==
% set pgf compatibility version
\pgfplotsset{compat=1.17}

% set path for \includegraphics
\graphicspath{{img/}}

\makeatletter
\newcommand{\IfPackageLoaded}[3]{\ltx@ifpackageloaded{#1}{#2}{#3}}
\makeatother

% set the width of epigraph quotes
\AtBeginDocument{%
    \IfPackageLoaded{natbib}{%
        \setlength{\epigraphwidth}{.65\textwidth}
    }{}
}

% use stars for nested itemize bullet points of level 2
\AtBeginDocument{%
    \IfPackageLoaded{enumitem}{%
        \renewcommand{\labelitemii}{$\star$}
    }{}
}

% make table header bold (when using \thead{})
\AtBeginDocument{%
    \IfPackageLoaded{makecell}{%
        \renewcommand\theadfont{\normalfont\bfseries}
    }{}
}

% break urls additionally on / - _
\def\UrlBreaks{\do\/\do-\do\_}

% set the padding of \fbox
\setlength\fboxsep{2pt}

% % patch acronyms to allow hyphenation
% % https://tex.stackexchange.com/a/69585/196218
% \makeatletter
% \patchcmd\@acf{\AC@acl}{\AC@foo}{}{}
% \patchcmd\@acf{\AC@acl}{\AC@foo}{}{}
% \patchcmd\@acf{\AC@foo}{\hskip\z@\AC@acl}{}{}
% \patchcmd\@acf{\AC@foo}{\hskip\z@\AC@acl}{}{}
% \makeatother

% \makeatletter
% \renewcommand*\AC@get[3]{%
%     \ifx#1\relax
%         \PackageWarning{acronym}{Acronym `#3' is not defined}%
%         \textbf{#3!}%
%     \else
%         \expandafter#2#1%
%     \fi}
% \makeatother


==> img/tikz/latex-common/tables/implementations-details.tex <==
{%
\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{ccc}
    \toprule
    \thead{Name} %
       & \thead{\acs{CCA}} %
       & \thead{HyStart} \\
    \midrule
    \makecell{\aioquic/} %
     & \makecell{\textbf{\NewReno/}} %
     & \makecell{\color{aluminium3}\faTimes} \\
    \makecell{\chrome/} %
     & \makecell{\BBRv2/, \CUBIC/} %
     & \makecell{\faCheck} \\
    \makecell{\kwik/} %
     & \makecell{\textbf{\NewReno/}} %
     & \makecell{\color{aluminium3}\faTimes} \\
    \makecell{\lsquic/} %
     & \makecell{\textbf{\BBR/}, \CUBIC/} %
     & \makecell{\color{aluminium3}\faTimes} \\
    \makecell{\msquic/} %
     & \makecell{\textbf{\CUBIC/}} %
     & \makecell{\color{aluminium3}\faTimes} \\
    \makecell{\mvfst/} %
     & \makecell{\BBR/, \textbf{\CUBIC/}, \NewReno/, \textellipsis} %
     & \makecell{\faCheck} \\
    \makecell{\neqo/} %
     & \makecell{\CUBIC/, \textbf{\NewReno/}} %
     & \makecell{\color{aluminium3}\faTimes} \\
    \makecell{\nginx/} %
     & \makecell{\color{aluminium5}\textcircled{?}} %
     & \makecell{\color{aluminium3}\faTimes} \\
    \makecell{\ngtcp/} %
     & \makecell{\BBRv2/, \BBR/, \textbf{\CUBIC/}, \Reno/} %
     & \makecell{\color{aluminium3}\faTimes} \\
    \makecell{\picoquic/} %
     & \makecell{\textbf{\BBR/}, \CUBIC/} %
     & \makecell{\faCheck} \\
    \makecell{\quant/} %
     & \makecell{\textbf{\NewReno/}} %
     & \makecell{\color{aluminium3}\faTimes} \\
    \makecell{\quicgo/} %
     & \makecell{\color{aluminium5}\CUBIC/ \textcircled{?}, \Reno/ \textcircled{?}} %
     & \makecell{\color{aluminium3}\faTimes} \\
    \makecell{\quiche/} %
     & \makecell{\textbf{\CUBIC/}} %
     & \makecell{\faCheck} \\
    \makecell{\quicly/} %
     & \makecell{\CUBIC/, \textbf{\Reno/}, \pico/} %
     & \makecell{\color{aluminium3}\faTimes} \\
    \makecell{\xquic/} %
     & \makecell{\textbf{\BBR/}, \CUBIC/, \Reno/} %
     & \makecell{\color{aluminium3}\faTimes} \\
    \arrayrulecolor{black}\bottomrule
\end{tabular}
}


==> img/tikz/latex-common/tables/implementations.tex <==
{%
\renewcommand{\arraystretch}{1.2}%
\begin{tabular}{cccc}
    \toprule
    \thead{Name} %
       & \thead{Role} %
       & \thead{Repository on GitHub / \URL/} %
       & \thead{Version} \\
    \midrule
    \makecell{\aioquic/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/aiortc/aioquic}{\texttt{aiortc/aioquic}}} %
     & \makecell{\small\color{aluminium5}0.9.17} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\chrome/} %
     & \makecell{client} %
     & \makecell{\href{https://github.com/marten-seemann/chrome-quic-interop-runner}{\texttt{marten-seemann/}}\\\href{https://github.com/marten-seemann/chrome-quic-interop-runner}{\texttt{chrome-quic-interop-runner}}} %
     & \makecell{\small\color{aluminium5}ChromeDriver\\\small\color{aluminium5}89.0.4389.23} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\kwik/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/ptrd/kwik}{\texttt{ptrd/kwik}}} %
     & \makecell{\small\color{aluminium5}\href{https://github.com/ptrd/kwik/commit/a9e478c}{\texttt{@a9e478c}}\\\small\color{aluminium5}(Nov 2021, 03)} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\lsquic/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/litespeedtech/lsquic}{\texttt{litespeedtech/lsquic}}} %
     & \makecell{\small\color{aluminium5}\textcircled{?}} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\msquic/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/microsoft/msquic}{\texttt{microsoft/msquic}}} %
     & \makecell{\small\color{aluminium5}\textcircled{?}} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\mvfst/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/facebookincubator/mvfst}{\texttt{facebookincubator/mvfst}}} %
     & \makecell{\small\color{aluminium5}\textcircled{?}} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\neqo/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/mozilla/neqo}{\texttt{mozilla/neqo}}} %
     & \makecell{\small\color{aluminium5}0.4.21} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\nginx/} %
     & \makecell{server} %
     & \makecell{\href{https://quic.nginx.org/}{\texttt{https://quic.nginx.org/}}} %
     & \makecell{\small\color{aluminium5}1.21.4} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\ngtcp/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/ngtcp2/ngtcp2}{\texttt{ngtcp2/ngtcp2}}} %
     & \makecell{\small\color{aluminium5}0.1.0-DEV \textcircled{?}} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\picoquic/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/private-octopus/picoquic}{\texttt{private-octopus/picoquic}}} %
     & \makecell{\small\color{aluminium5}\href{https://github.com/private-octopus/picoquic/commit/8dfc4776}{\texttt{@8dfc4776}}\\\small\color{aluminium5}(Oct 2021, 23)} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\quant/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/NTAP/quant}{\texttt{NTAP/quant}}} %
     & \makecell{\small\color{aluminium5}0.0.34 \textcircled{?}} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\quicgo/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/lucas-clemente/quic-go}{\texttt{lucas-clemente/quic-go}}} %
     & \makecell{\small\color{aluminium5}0.23.0} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\quiche/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/cloudflare/quiche}{\texttt{cloudflare/quiche}}} %
     & \makecell{\small\color{aluminium5}\textcircled{?}} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\quicly/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/h2o/quicly}{\texttt{h2o/quicly}}} %
     & \makecell{\small\color{aluminium5}\href{https://github.com/h2o/quicly/commit/699e2564}{\texttt{@699e2564}}\\\small\color{aluminium5}(Nov 2021, 10)} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\xquic/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/Kulsk/xquic}{\texttt{Kulsk/xquic}}} %
     & \makecell{\small\color{aluminium5}\textcircled{?}} \\
    \arrayrulecolor{black}\bottomrule
\end{tabular}
}


==> img/tikz/latex-common/tables/rel_results_table.tex <==
{%
\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{cccccccc}
    \toprule
    \thead{Source} %
       & \thead{Imple-\\men-\\tation} %
       & \thead{Link\\Rate} %
       & \thead{\RTT/} %
       & \thead{\acs{PLR}} %
       & \thead{Size\\} %
       & \thead{\acs{PLT} /\\\acs{TTLB}\\} %
       & \thead{Good-\\put\\}  \\
    % no unit
       & % no unit
       & \makecell{\makeunit{\mbps}} %
       & \makecell{\makeunit{\milli\second}} %
       & % no unit
       & \makecell{\makeunit{\mib}} %
       & \makecell{\makeunit{\second}} %
       & \makecell{\makeunit{\mbps}} \\
    \midrule
    \multirow[c]{2}{*}{\makecell{Jones\\2021~\cite{jonesEnhancingTransportProtocols2021}}} %
     & \makecell{\color{aluminium3}\textcircled{?}} %
     & \makecell{50\color{aluminium4}/10} %
     & \makecell{650} %
     & \makecell{\color{aluminium3}---} %
     & \makecell{10} %
     & \makecell{5.0} %
     & \makecell{16.78} \\
       % multirow %
     & \makecell{\color{aluminium3}\textcircled{?}} %
     & \makecell{10\color{aluminium4}/2} %
     & \makecell{650} %
     & \makecell{\color{aluminium3}---} %
     & \makecell{10} %
     & \makecell{10.0} %
     & \makecell{8.39} \\
    \arrayrulecolor{aluminium2}\hline
    \multirow[c]{3}{*}{\makecell{\hyperref[sec:review_f]{\textcircled{F}}\\Deutschmann\\2019~\cite{deutschmannSatelliteInternetPerformance2019}}} %
     & \makecell{\chrome/} %
     & \makecell{20\color{aluminium4}/2} %
     & \multicolumn{2}{c}{\makecell{\color{aluminium3}\textit{real Link}}} %
     & % multicol
       \makecell{10~\textsuperscript{\color{aluminium4}\faFile}} %
     & \makecell{75.0} %
     & \makecell{1.12} \\
       % multirow %
     & \makecell{\chrome/} %
     & \makecell{30\color{aluminium4}/2} %
     & \multicolumn{2}{c}{\makecell{\color{aluminium3}\textit{real Link}}} %
     & % multicol
       \makecell{10~\textsuperscript{\color{aluminium4}\faFile}} %
     & \makecell{73.0} %
     & \makecell{1.15} \\
       % multirow %
     & \makecell{\chrome/} %
     & \makecell{15\color{aluminium4}/3} %
     & \multicolumn{2}{c}{\makecell{\color{aluminium3}\textit{real Link}}} %
     & % multicol
       \makecell{10~\textsuperscript{\color{aluminium4}\faFile}} %
     & \makecell{15.0} %
     & \makecell{5.59} \\
    \arrayrulecolor{aluminium2}\hline
    \multirow[c]{1}{*}{\makecell{\hyperref[sec:review_i]{\textcircled{I}} Mogildea\\2019~\cite{mogildeaQUICSatelliteIntroduction2019}}} %
     & \makecell{\ngtcp/} %
     & \makecell{20\color{aluminium4}/2} %
     & \multicolumn{2}{c}{\makecell{\color{aluminium3}\textit{real Link}}} %
     & % multicol
       \makecell{1} %
     & \makecell{8.5} %
     & \makecell{0.99} \\
       % multirow %
     & \makecell{\ngtcp/} %
     & \makecell{20\color{aluminium4}/2} %
     & \makecell{600} %
     & \makecell{\color{aluminium5}\SI{0}{\percent}} %
     & \makecell{1} %
     & \makecell{8.0} %
     & \makecell{1.05} \\
    \arrayrulecolor{black}\bottomrule
\end{tabular}
}


==> img/tikz/latex-common/tables/rel_work_table.tex <==
{%
\renewcommand{\arraystretch}{2}%
\begin{tabular}{cccccc}
    \toprule
    \thead{Reference} %
         & \thead{\QUIC/\\Version} %
         & \thead{Client} %
         & \thead{Server} %
         & \thead{Type of\\Benchmark} %
         & \thead{Type of\\Link} \\
    \midrule
    \makecell{\hyperref[sec:review_a]{\textcircled{A}} Rula\\2018~\cite{rulaMileHighWiFi2018}} %
     & \makecell{\textcircled{?}} %
     & \makecell{\textcircled{?}} %
     & \makecell{\textcircled{?}} %
     & \makecell{Websites} %
     & \makecell{emul.} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_b]{\textcircled{B}} Yang\\2018~\cite{yangPerformanceAnalysisQUIC2018}} %
     & \makecell{\texttt{\gQUIC/}\\\texttt{Q035}} %
     & \makecell{\chrome/} %
     & \makecell{\quicgo/} %
     & \makecell{Website} %
     & \makecell{emul.} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_c]{\textcircled{C}} Zhang\\2018~\cite{zhangHowQuickQUIC2018}} %
     & \makecell{\texttt{\gQUIC/}\\\texttt{Q039}} %
     & \makecell{\chrome/} %
     & \makecell{Google QUIC\\test server} %
     & \makecell{Websites} %
     & \makecell{emul.} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_d]{\textcircled{D}} Wang\\2018~\cite{wangPerformanceEvaluationQUIC2018}} %
     & \makecell{\texttt{\gQUIC/}\\\texttt{Q039}} %
     & \makecell{\chrome/} %
     & \makecell{Google QUIC\\test server} %
     & \makecell{Websites} %
     & \makecell{emul.} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_e]{\textcircled{E}} Thomas\\2019~\cite{thomasGoogleQUICPerformance2019}} %
     & \makecell{\texttt{\gQUIC/}\\\texttt{Q039}} %
     & \makecell{\chrome/\\67} %
     & \makecell{Google\\Server} %
     & \makecell{File} %
     & \makecell{real} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_f]{\textcircled{F}} Deutsch-\\mann\\2019~\cite{deutschmannSatelliteInternetPerformance2019}} %
     & \makecell{\texttt{\gQUIC/}\\\texttt{Q043}} %
     & \makecell{\chrome/\\69} %
     & \makecell{\chrome/\\\quicgo/} %
     & \makecell{File} %
     & \makecell{real} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_g]{\textcircled{G}} Fairhurst\\2019~\cite{fairhurstMeasuringQUICDynamics2019}} %
     & \makecell{\texttt{draft-20}} %
     & \multicolumn{2}{c}{\makecell{\quicly/ v20}} %
     & \makecell{Files} %
     & \makecell{real} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_h]{\textcircled{H}} Wolsing\\2019~\cite{wolsingPerformancePerspectiveWeb2019}} %
     & \makecell{\texttt{\gQUIC/}\\\texttt{Q043}} %
     & \makecell{\chrome/\\70} %
     & \makecell{Google QUIC\\test server} %
     & \makecell{real\\Websites} %
     & \makecell{emul.} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_i]{\textcircled{I}} Mogildea\\2019~\cite{mogildeaQUICSatelliteIntroduction2019}} %
     & \makecell{\texttt{Q046}\\\texttt{draft-22}\\\texttt{draft-22}} %
     & \multicolumn{2}{c}{\makecell{\chrome/\\\quicly/\\\ngtcp/}} %
     & \makecell{File} %
     & \makecell{real,\\emul.} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_j]{\textcircled{J}} Border\\2020~\cite{borderEvaluatingQUICPerformance2020}} %
     & \makecell{\texttt{\gQUIC/}\\\texttt{Q046}} %
     & \makecell{\chrome/\\77} %
     & \makecell{Google\\Drive} %
     & \makecell{File} %
     & \makecell{real,\\emul.} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_k]{\textcircled{K}} Kuhn\\2020~\cite{kuhnQUICOpportunitiesThreats2020}} %
     & \makecell{\texttt{\gQUIC/}\\\textcircled{?}} %
     & \makecell{\chrome/\\67} %
     & \makecell{Google\\Server} %
     & \makecell{Websites} %
     & \makecell{real} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_l]{\textcircled{L}} Custura\\2020~\cite{custuraImpactAcknowledgementsUsing2020}} %
     & \makecell{\texttt{draft-27}\\\texttt{draft-26}} %
     & \multicolumn{2}{c}{\makecell{\quicly/\\\chrome/}} %
     & \makecell{File} %
     & \makecell{real,\\emul.} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_m]{\textcircled{M}} Kuhn\\2021~\cite{kuhnFeedbackUsingQUIC2021}} %
     & \makecell{\textcircled{?}} %
     & \multicolumn{2}{c}{\makecell{\picoquic/}} %
     & \makecell{File} %
     & \makecell{emul.} \\
    \arrayrulecolor{black}\bottomrule
\end{tabular}
}


==> img/tikz/latex-common/tables/results-table.tex <==
{%
\begin{tabular}{ccccccc}
    \toprule
    \thead{Measurement} %
       & \multicolumn{2}{c}{\thead{Mean}} %
       & % multicol
         \multicolumn{2}{c}{\thead{Maximum}} %
       & % multicol
         \thead{Failed} %
       & \thead{Timeout}  \\
    % no unit
       & \makecell{\makeunit{\mbps}} %
       & \makecell{\makeunit{\percent}} %
       & \makecell{\makeunit{\mbps}} %
       & \makecell{\makeunit{\percent}} %
       & \makecell{\makeunit{\percent}} %
       & \makecell{\makeunit{\percent}} \\
    \midrule
    \makecell{\g/} %
     & \cellcolor{Chameleon!40}8.54 %
     & \cellcolor{Chameleon!40}85 %
     & \cellcolor{ScarletRed!40}9.6 %
     & \cellcolor{Chameleon!40}96 %
     & \cellcolor{LightScarletRed!15}35 %
     & \cellcolor{LightOrange!10}7 \\
    \makecell{\sat/} %
     & \cellcolor{LightScarletRed!15}4.88 %
     & \cellcolor{LightScarletRed!15}24 %
     & \cellcolor{LightScarletRed!15}12.0 %
     & \cellcolor{LightOrange!10}60 %
     & \cellcolor{DarkOrange!10}28 %
     & \cellcolor{LightChameleon!15}3 \\
    \makecell{\satl/} %
     & \cellcolor{ScarletRed!40}2.86 %
     & \cellcolor{ScarletRed!20}14 %
     & \cellcolor{ScarletRed!20}11.5 %
     & \cellcolor{Orange!5}57 %
     & \cellcolor{ScarletRed!40}44 %
     & \cellcolor{DarkOrange!10}10 \\
    \makecell{\astra/} %
     & \cellcolor{ScarletRed!20}3.98 %
     & \cellcolor{ScarletRed!20}20 %
     & \cellcolor{DarkOrange!10}13.5 %
     & \cellcolor{LightOrange!10}68 %
     & \cellcolor{ScarletRed!40}51 %
     & \cellcolor{ScarletRed!40}18 \\
    \makecell{\eut/} %
     & \cellcolor{Orange!5}6.01 %
     & \cellcolor{ScarletRed!20}12 %
     & \cellcolor{Chameleon!40}17.5 %
     & \cellcolor{LightScarletRed!15}35 %
     & \cellcolor{ScarletRed!40}45 %
     & \cellcolor{ScarletRed!20}16 \\
    \arrayrulecolor{black}\bottomrule
\end{tabular}
}


==> img/tikz/latex-common/tables/scenarios.tex <==
{%
\renewcommand{\arraystretch}{1.3}%
\begin{tabular}{cccccccc}
    \toprule
    \thead{Name} %
       & \thead{\RTT/} %
       & \thead{Data\\Rate} %
       & \thead{\acs{PLR}} %
       & \thead{Time-\\out} %
       & \thead{Min.\\Goodput} %
       & \thead{Min.\\Efficiency} %
       & \thead{\acs{BDP}}  \\
    % no unit
       & \makecell{\makeunit{\milli\second}} %
       & \makecell{\makeunit{\mbps}} %
       & \makecell{\makeunit{\percent}} %
       & \makecell{\makeunit{\second}} %
       & \makecell{\makeunit{\mbps}} %
       & \makecell{\makeunit{\percent}} %
       & \makecell{\makeunit{\mib}} \\
    \midrule
    \makecell{\lr/} %
     & \makecell{1500} %
     & \makecell{10} %
     & \makecell{\color{aluminium5}0} %
     & \makecell{60} %
     & \makecell{\color{aluminium3}---} %
     & \makecell{\color{aluminium3}---} %
     & \makecell{7.2} \\
    \makecell{\g/} %
     & \makecell{30} %
     & \makecell{10} %
     & \makecell{\color{aluminium5}0} %
     & \makecell{60} %
     & \makecell{1.4} %
     & \makecell{14} %
     & \makecell{0.1} \\
    \makecell{\sat/} %
     & \makecell{600} %
     & \makecell{20/2} %
     & \makecell{\color{aluminium5}0} %
     & \makecell{120} %
     & \makecell{0.7} %
     & \makecell{3} %
     & \makecell{5.7} \\
    \makecell{\satl/} %
     & \makecell{600} %
     & \makecell{20/2} %
     & \makecell{1} %
     & \makecell{360} %
     & \makecell{0.2} %
     & \makecell{1} %
     & \makecell{5.7} \\
    \makecell{\astra/} %
     & \makecell{\color{aluminium4}$\gtrapprox$600} %
     & \makecell{\color{aluminium5}20/2} %
     & \makecell{\color{aluminium4}$\lessapprox$0.1} %
     & \makecell{120} %
     & \makecell{0.7} %
     & \makecell{3} %
     & \makecell{5.7} \\
    \makecell{\eut/} %
     & \makecell{\color{aluminium4}$\gtrapprox$600} %
     & \makecell{\color{aluminium5}50/5} %
     & \makecell{\color{aluminium4}$\lessapprox$0.1} %
     & \makecell{120} %
     & \makecell{0.7} %
     & \makecell{1} %
     & \makecell{14.3} \\
    \arrayrulecolor{black}\bottomrule
\end{tabular}
}


==> img/tikz/latex-common/tikz-cmds.tex <==
\newcommand{\vertCurledArrow}[4]{%
    \draw[#1] (#3.east) .. controls ([xshift=#2]#3.east) and ([xshift=-#2]#4.west) .. (#4.west);
}

\newcommand{\satellite}[3]{%
    \begin{scope}[shift={#1}, rotate=#2, scale=#3]
        \draw[sat] (-4mm,-4mm) rectangle (4mm,4mm);
        \draw[sat] (-2mm,5mm) rectangle (2mm,15mm);
        \draw[sat] (-2mm,-15mm) rectangle (2mm,-5mm);
        \filldraw[sat] (-6mm,4mm) -- (-6mm,-4mm) arc(-45:45:5.657mm) (-6mm,4mm);
    \end{scope}
}


==> img/tikz/latex-common/tikz-setup.tex <==
\usepackage{pgfplots}

\usetikzlibrary{animations}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{arrows}
\usetikzlibrary{backgrounds}
\usetikzlibrary{calc}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{external}
\usetikzlibrary{fadings}
\usetikzlibrary{fit}
\usetikzlibrary{matrix}
\usetikzlibrary{patterns}
\usetikzlibrary{positioning}
\usetikzlibrary{shadows}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{shapes.misc}
\usetikzlibrary{shapes.multipart}
\usetikzlibrary{shapes}

==> latex-common/tables/implementations.tex <==
{%
\renewcommand{\arraystretch}{1.2}%
\begin{tabular}{cccc}
    \toprule
    \thead{Name} %
       & \thead{Role} %
       & \thead{Repository on GitHub / \URL/} %
       & \thead{Version} \\
    \midrule
    \makecell{\aioquic/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/aiortc/aioquic}{\texttt{aiortc/aioquic}}} %
     & \makecell{\small\color{aluminium5}0.9.17} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\chrome/} %
     & \makecell{client} %
     & \makecell{\href{https://github.com/marten-seemann/chrome-quic-interop-runner}{\texttt{marten-seemann/}}\\\href{https://github.com/marten-seemann/chrome-quic-interop-runner}{\texttt{chrome-quic-interop-runner}}} %
     & \makecell{\small\color{aluminium5}ChromeDriver\\\small\color{aluminium5}89.0.4389.23} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\kwik/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/ptrd/kwik}{\texttt{ptrd/kwik}}} %
     & \makecell{\small\color{aluminium5}\href{https://github.com/ptrd/kwik/commit/a9e478c}{\texttt{@a9e478c}}\\\small\color{aluminium5}(Nov 2021, 03)} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\lsquic/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/litespeedtech/lsquic}{\texttt{litespeedtech/lsquic}}} %
     & \makecell{\small\color{aluminium5}\textcircled{?}} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\msquic/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/microsoft/msquic}{\texttt{microsoft/msquic}}} %
     & \makecell{\small\color{aluminium5}\textcircled{?}} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\mvfst/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/facebookincubator/mvfst}{\texttt{facebookincubator/mvfst}}} %
     & \makecell{\small\color{aluminium5}\textcircled{?}} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\neqo/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/mozilla/neqo}{\texttt{mozilla/neqo}}} %
     & \makecell{\small\color{aluminium5}0.4.21} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\nginx/} %
     & \makecell{server} %
     & \makecell{\href{https://quic.nginx.org/}{\texttt{https://quic.nginx.org/}}} %
     & \makecell{\small\color{aluminium5}1.21.4} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\ngtcp/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/ngtcp2/ngtcp2}{\texttt{ngtcp2/ngtcp2}}} %
     & \makecell{\small\color{aluminium5}0.1.0-DEV \textcircled{?}} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\picoquic/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/private-octopus/picoquic}{\texttt{private-octopus/picoquic}}} %
     & \makecell{\small\color{aluminium5}\href{https://github.com/private-octopus/picoquic/commit/8dfc4776}{\texttt{@8dfc4776}}\\\small\color{aluminium5}(Oct 2021, 23)} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\quant/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/NTAP/quant}{\texttt{NTAP/quant}}} %
     & \makecell{\small\color{aluminium5}0.0.34 \textcircled{?}} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\quicgo/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/lucas-clemente/quic-go}{\texttt{lucas-clemente/quic-go}}} %
     & \makecell{\small\color{aluminium5}0.23.0} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\quiche/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/cloudflare/quiche}{\texttt{cloudflare/quiche}}} %
     & \makecell{\small\color{aluminium5}\textcircled{?}} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\quicly/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/h2o/quicly}{\texttt{h2o/quicly}}} %
     & \makecell{\small\color{aluminium5}\href{https://github.com/h2o/quicly/commit/699e2564}{\texttt{@699e2564}}\\\small\color{aluminium5}(Nov 2021, 10)} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\xquic/} %
     & \makecell{\color{aluminium3}both} %
     & \makecell{\href{https://github.com/Kulsk/xquic}{\texttt{Kulsk/xquic}}} %
     & \makecell{\small\color{aluminium5}\textcircled{?}} \\
    \arrayrulecolor{black}\bottomrule
\end{tabular}
}


==> latex-common/tables/rel_results_table.tex <==
{%
\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{cccccccc}
    \toprule
    \thead{Source} %
       & \thead{Imple-\\men-\\tation} %
       & \thead{Link\\Rate} %
       & \thead{\RTT/} %
       & \thead{\acs{PLR}} %
       & \thead{Size\\} %
       & \thead{\acs{PLT} /\\\acs{TTLB}\\} %
       & \thead{Good-\\put\\}  \\
    % no unit
       & % no unit
       & \makecell{\makeunit{\mbps}} %
       & \makecell{\makeunit{\milli\second}} %
       & % no unit
       & \makecell{\makeunit{\mib}} %
       & \makecell{\makeunit{\second}} %
       & \makecell{\makeunit{\mbps}} \\
    \midrule
    \multirow[c]{2}{*}{\makecell{Jones\\2021~\cite{jonesEnhancingTransportProtocols2021}}} %
     & \makecell{\color{aluminium3}\textcircled{?}} %
     & \makecell{50\color{aluminium4}/10} %
     & \makecell{650} %
     & \makecell{\color{aluminium3}---} %
     & \makecell{10} %
     & \makecell{5.0} %
     & \makecell{16.78} \\
       % multirow %
     & \makecell{\color{aluminium3}\textcircled{?}} %
     & \makecell{10\color{aluminium4}/2} %
     & \makecell{650} %
     & \makecell{\color{aluminium3}---} %
     & \makecell{10} %
     & \makecell{10.0} %
     & \makecell{8.39} \\
    \arrayrulecolor{aluminium2}\hline
    \multirow[c]{3}{*}{\makecell{\hyperref[sec:review_f]{\textcircled{F}}\\Deutschmann\\2019~\cite{deutschmannSatelliteInternetPerformance2019}}} %
     & \makecell{\chrome/} %
     & \makecell{20\color{aluminium4}/2} %
     & \multicolumn{2}{c}{\makecell{\color{aluminium3}\textit{real Link}}} %
     & % multicol
       \makecell{10~\textsuperscript{\color{aluminium4}\faFile}} %
     & \makecell{75.0} %
     & \makecell{1.12} \\
       % multirow %
     & \makecell{\chrome/} %
     & \makecell{30\color{aluminium4}/2} %
     & \multicolumn{2}{c}{\makecell{\color{aluminium3}\textit{real Link}}} %
     & % multicol
       \makecell{10~\textsuperscript{\color{aluminium4}\faFile}} %
     & \makecell{73.0} %
     & \makecell{1.15} \\
       % multirow %
     & \makecell{\chrome/} %
     & \makecell{15\color{aluminium4}/3} %
     & \multicolumn{2}{c}{\makecell{\color{aluminium3}\textit{real Link}}} %
     & % multicol
       \makecell{10~\textsuperscript{\color{aluminium4}\faFile}} %
     & \makecell{15.0} %
     & \makecell{5.59} \\
    \arrayrulecolor{aluminium2}\hline
    \multirow[c]{1}{*}{\makecell{\hyperref[sec:review_i]{\textcircled{I}} Mogildea\\2019~\cite{mogildeaQUICSatelliteIntroduction2019}}} %
     & \makecell{\ngtcp/} %
     & \makecell{20\color{aluminium4}/2} %
     & \multicolumn{2}{c}{\makecell{\color{aluminium3}\textit{real Link}}} %
     & % multicol
       \makecell{1} %
     & \makecell{8.5} %
     & \makecell{0.99} \\
       % multirow %
     & \makecell{\ngtcp/} %
     & \makecell{20\color{aluminium4}/2} %
     & \makecell{600} %
     & \makecell{\color{aluminium5}\SI{0}{\percent}} %
     & \makecell{1} %
     & \makecell{8.0} %
     & \makecell{1.05} \\
    \arrayrulecolor{black}\bottomrule
\end{tabular}
}


==> latex-common/tables/rel_work_table.tex <==
{%
\renewcommand{\arraystretch}{2}%
\begin{tabular}{cccccc}
    \toprule
    \thead{Reference} %
         & \thead{\QUIC/\\Version} %
         & \thead{Client} %
         & \thead{Server} %
         & \thead{Type of\\Benchmark} %
         & \thead{Type of\\Link} \\
    \midrule
    \makecell{\hyperref[sec:review_a]{\textcircled{A}} Rula\\2018~\cite{rulaMileHighWiFi2018}} %
     & \makecell{\textcircled{?}} %
     & \makecell{\textcircled{?}} %
     & \makecell{\textcircled{?}} %
     & \makecell{Websites} %
     & \makecell{emul.} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_b]{\textcircled{B}} Yang\\2018~\cite{yangPerformanceAnalysisQUIC2018}} %
     & \makecell{\texttt{\gQUIC/}\\\texttt{Q035}} %
     & \makecell{\chrome/} %
     & \makecell{\quicgo/} %
     & \makecell{Website} %
     & \makecell{emul.} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_c]{\textcircled{C}} Zhang\\2018~\cite{zhangHowQuickQUIC2018}} %
     & \makecell{\texttt{\gQUIC/}\\\texttt{Q039}} %
     & \makecell{\chrome/} %
     & \makecell{Google QUIC\\test server} %
     & \makecell{Websites} %
     & \makecell{emul.} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_d]{\textcircled{D}} Wang\\2018~\cite{wangPerformanceEvaluationQUIC2018}} %
     & \makecell{\texttt{\gQUIC/}\\\texttt{Q039}} %
     & \makecell{\chrome/} %
     & \makecell{Google QUIC\\test server} %
     & \makecell{Websites} %
     & \makecell{emul.} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_e]{\textcircled{E}} Thomas\\2019~\cite{thomasGoogleQUICPerformance2019}} %
     & \makecell{\texttt{\gQUIC/}\\\texttt{Q039}} %
     & \makecell{\chrome/\\67} %
     & \makecell{Google\\Server} %
     & \makecell{File} %
     & \makecell{real} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_f]{\textcircled{F}} Deutsch-\\mann\\2019~\cite{deutschmannSatelliteInternetPerformance2019}} %
     & \makecell{\texttt{\gQUIC/}\\\texttt{Q043}} %
     & \makecell{\chrome/\\69} %
     & \makecell{\chrome/\\\quicgo/} %
     & \makecell{File} %
     & \makecell{real} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_g]{\textcircled{G}} Fairhurst\\2019~\cite{fairhurstMeasuringQUICDynamics2019}} %
     & \makecell{\texttt{draft-20}} %
     & \multicolumn{2}{c}{\makecell{\quicly/ v20}} %
     & \makecell{Files} %
     & \makecell{real} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_h]{\textcircled{H}} Wolsing\\2019~\cite{wolsingPerformancePerspectiveWeb2019}} %
     & \makecell{\texttt{\gQUIC/}\\\texttt{Q043}} %
     & \makecell{\chrome/\\70} %
     & \makecell{Google QUIC\\test server} %
     & \makecell{real\\Websites} %
     & \makecell{emul.} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_i]{\textcircled{I}} Mogildea\\2019~\cite{mogildeaQUICSatelliteIntroduction2019}} %
     & \makecell{\texttt{Q046}\\\texttt{draft-22}\\\texttt{draft-22}} %
     & \multicolumn{2}{c}{\makecell{\chrome/\\\quicly/\\\ngtcp/}} %
     & \makecell{File} %
     & \makecell{real,\\emul.} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_j]{\textcircled{J}} Border\\2020~\cite{borderEvaluatingQUICPerformance2020}} %
     & \makecell{\texttt{\gQUIC/}\\\texttt{Q046}} %
     & \makecell{\chrome/\\77} %
     & \makecell{Google\\Drive} %
     & \makecell{File} %
     & \makecell{real,\\emul.} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_k]{\textcircled{K}} Kuhn\\2020~\cite{kuhnQUICOpportunitiesThreats2020}} %
     & \makecell{\texttt{\gQUIC/}\\\textcircled{?}} %
     & \makecell{\chrome/\\67} %
     & \makecell{Google\\Server} %
     & \makecell{Websites} %
     & \makecell{real} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_l]{\textcircled{L}} Custura\\2020~\cite{custuraImpactAcknowledgementsUsing2020}} %
     & \makecell{\texttt{draft-27}\\\texttt{draft-26}} %
     & \multicolumn{2}{c}{\makecell{\quicly/\\\chrome/}} %
     & \makecell{File} %
     & \makecell{real,\\emul.} \\\arrayrulecolor{aluminium2}\hline
    \makecell{\hyperref[sec:review_m]{\textcircled{M}} Kuhn\\2021~\cite{kuhnFeedbackUsingQUIC2021}} %
     & \makecell{\textcircled{?}} %
     & \multicolumn{2}{c}{\makecell{\picoquic/}} %
     & \makecell{File} %
     & \makecell{emul.} \\
    \arrayrulecolor{black}\bottomrule
\end{tabular}
}


==> latex-common/tables/scenarios.tex <==
{%
\renewcommand{\arraystretch}{1.3}%
\begin{tabular}{cccccccc}
    \toprule
    \thead{Name} %
       & \thead{\RTT/} %
       & \thead{Data\\Rate} %
       & \thead{\acs{PLR}} %
       & \thead{Time-\\out} %
       & \thead{Min.\\Goodput} %
       & \thead{Min.\\Efficiency} %
       & \thead{\acs{BDP}}  \\
    % no unit
       & \makecell{\makeunit{\milli\second}} %
       & \makecell{\makeunit{\mbps}} %
       & \makecell{\makeunit{\percent}} %
       & \makecell{\makeunit{\second}} %
       & \makecell{\makeunit{\mbps}} %
       & \makecell{\makeunit{\percent}} %
       & \makecell{\makeunit{\mib}} \\
    \midrule
    \makecell{\lr/} %
     & \makecell{1500} %
     & \makecell{10} %
     & \makecell{\color{aluminium5}0} %
     & \makecell{60} %
     & \makecell{\color{aluminium3}---} %
     & \makecell{\color{aluminium3}---} %
     & \makecell{7.2} \\
    \makecell{\g/} %
     & \makecell{30} %
     & \makecell{10} %
     & \makecell{\color{aluminium5}0} %
     & \makecell{60} %
     & \makecell{1.4} %
     & \makecell{14} %
     & \makecell{0.1} \\
    \makecell{\sat/} %
     & \makecell{600} %
     & \makecell{20/2} %
     & \makecell{\color{aluminium5}0} %
     & \makecell{120} %
     & \makecell{0.7} %
     & \makecell{3} %
     & \makecell{5.7} \\
    \makecell{\satl/} %
     & \makecell{600} %
     & \makecell{20/2} %
     & \makecell{1} %
     & \makecell{360} %
     & \makecell{0.2} %
     & \makecell{1} %
     & \makecell{5.7} \\
    \makecell{\astra/} %
     & \makecell{\color{aluminium4}$\gtrapprox$600} %
     & \makecell{\color{aluminium5}20/2} %
     & \makecell{\color{aluminium4}$\lessapprox$0.1} %
     & \makecell{120} %
     & \makecell{0.7} %
     & \makecell{3} %
     & \makecell{5.7} \\
    \makecell{\eut/} %
     & \makecell{\color{aluminium4}$\gtrapprox$600} %
     & \makecell{\color{aluminium5}50/5} %
     & \makecell{\color{aluminium4}$\lessapprox$0.1} %
     & \makecell{120} %
     & \makecell{0.7} %
     & \makecell{1} %
     & \makecell{14.3} \\
    \arrayrulecolor{black}\bottomrule
\end{tabular}
}

